Exactly solving the KPZ equation

We present a complete proof of the exact formula for the one-point distribution for the narrow-wedge Hopf-Cole solution to the Kardar-Parisi-Zhang (KPZ) equation. This presentation is intended to be self-contained so no previous knowledge about stochastic PDEs, or exactly solvable systems is presumed.

==> macros.tex <==
%    If you need symbols beyond the basic set, uncomment this command.
\usepackage{amssymb}

%    If your article includes graphics, uncomment this command.
%\usepackage{graphicx}

%    If the article includes commutative diagrams, ...
%\usepackage[cmtip,all]{xy}

%    Include other referenced packages here.
\usepackage{amsmath,amsthm,tikz,mathrsfs,pgfplots,enumerate}
\usepackage{bm}
%\usepackage{subfiles}
\RequirePackage[numbers,sort&compress]{natbib}
\RequirePackage{color}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\RequirePackage[colorlinks, urlcolor=my-blue,linkcolor=my-link,citecolor=my-green]{hyperref}
%\usepackage[colorlinks=true]{hyperref}
%the link colors were adjusted slightly so that they print nicely even in black and white

%\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
%\usepackage[left=1.5in,top=1.5in,right=1.5in,bottom=1.4in]{geometry}

%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}

\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\renewcommand{\bibsection}{\section*{\refname}}

%Ivan's packages
\usepackage{bbm}
%\usepackage{amsfonts,amsbsy, amscd}
%\usepackage{graphicx,psfrag,subfigure} %,url}
%\usepackage{cite}
%\usepackage[DIV13]{typearea}
%\usepackage{comment}
%\usepackage{caption}
%\usepackage{setspace}
%\usepackage{float}

%\usepackage{chapterbib}
%\usepackage{minitoc}
%\usepackage{appendix}
%\setcounter{secnumdepth}{3}

%\usepackage{filemod} 
%\date{Last modified on \today\ at\ \filemodprinttime{\jobname}}
%\date{December 05, 2016}



%    Update the information and uncomment if AMS is not the copyright
%    holder.
%\copyrightinfo{2009}{American Mathematical Society}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{formal}[theorem]{Critical point derivation}
\newtheorem{experiment}[theorem]{Experimental Result}
\newtheorem{clam}[theorem]{Claim}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conj}[theorem]{Conjecture}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
\newtheorem{quest}{Question}


\allowdisplaybreaks[1]
\numberwithin{figure}{section}
\numberwithin{equation}{section}

\newcommand\docname[2]{#2}

\let\LATEXindex\index % save old definition to prevent recursion
\renewcommand\index[1]{\LATEXindex{#1|docname{\jobname}}}
\makeindex

%%%%%%%%%%%%%%%%%%%%
%Firas' macros
%%%%%%%%%%%%%%%%%%%%
\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{sussexb}{rgb}{0.4,0.4,0.7}
\definecolor{mygray}{rgb}{0.75,0.75,0.75}


\newcommand{\E}{\mathbb{E}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cT}{\mathcal{T}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\e}{\varepsilon}
\newcommand{\kS}{\mathfrak{S}}
\def\w{\omega}
\def\Bavg{\overline B}
\def\Gbar{\overline G}
\def\cid{\xi^*}

\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\riUset{\Uset^\circ}

\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}    %indicator function

\def\thick{2pt}



%%%%%%%%%%%%%%%%%%%%
%Timo's macros
%%%%%%%%%%%%%%%%%%%%
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}
\def\cC{\mathcal{C}}  \def\cD{\mathcal{D}}
\def\cR{\mathcal{R}}
\def\cU{\mathcal{U}}
\def\cK{\mathcal{K}}
\def\cX{\mathcal{X}}\def\cY{\mathcal{Y}}\def\cZ{\mathcal{Z}}
\def\bE{\mathbb{E}} \def\bL{\mathbb{L}}
\def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
\def\wvec{\mathbf{w}}
\def\ind{\mathbf{1}}
\def\ddd{\displaystyle} 
\def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
\def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}
\def\north{S_{\mathcal N}}  \def\south{S_{\mathcal S}}  \def\east{S_{\mathcal E}}  
\def\west{S_{\mathcal W}}  
\def\OSP{(\Omega, \kS, \P)}
\def\Gpl{G}
\def\Gpp{G}
\def\gpp{g_{\text{\rm pp}}}
\def\gpl{g_{\text{\rm pl}}}  
\def\B{{B}}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\conv}{co}   %convex hull  
\def\sigmawc{\wc\sigma}   %sigma check (needed version that doesn't start \w...  
\def\loexp{\chi}  %longitudinal exponent
\def\trexp{\zeta}  %transverse exponent
\def\deq{\overset{d}=} 
\def\qedex{\hfill$\triangle$} 
\def\bincr{B}   \def\tincr{t}   \def\Iincr{I}
\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\ul{\underline}  
\def\exitt{\tau} %exit time from axis 
\def\Gppo{{{}^o\Gpp}}
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\bbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}
\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up


%%%%%%%%%%%%%%%%%%%%
%Ivan's macros
%%%%%%%%%%%%%%%%%%%%
\newcommand{\bflambda}{\ensuremath{\bar{\lambda}}}
\newcommand{\bfmu}{\ensuremath{\bar{\mu}}}
\newcommand{\bfnu}{\ensuremath{\bar{\nu}}}
\newcommand{\I}{{\rm i}}
\newcommand{\Id}{\mathbbm{1}}
\newcommand{\Or}{\mathcal{O}}
%\newcommand{\e}[0]{\varepsilon}
\newcommand{\BesselK}{\ensuremath{\mathrm{K}}}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
%\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
%\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Rplus}{\ensuremath{\mathbb{R}_{+}}}
\newcommand{\Zgzero}{\ensuremath{\mathbb{Z}_{>0}}}
\newcommand{\Zgeqzero}{\ensuremath{\mathbb{Z}_{\geq 0}}}
\newcommand{\Zleqzero}{\ensuremath{\mathbb{Z}_{\leq 0}}}
%\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\M}{\ensuremath{\mathbf{M}}}
\newcommand{\MM}{\ensuremath{\mathbf{MM}}}
\newcommand{\W}[1]{\ensuremath{\mathbf{W}}_{(#1)}}
\newcommand{\WM}[1]{\ensuremath{\mathbf{WM}}_{(#1)}}
\newcommand{\Zsd}{\ensuremath{\mathbf{Z}}}
\newcommand{\Fsd}{\ensuremath{\mathbf{F}}}
\newcommand{\Usd}{\ensuremath{\mathbf{U}}}
\newcommand{\Sym}{\ensuremath{\mathrm{Sym}}}
\newcommand{\Gdist}{\ensuremath{\mathrm{Gamma}}}
\newcommand{\LogGdist}{\ensuremath{\log\Gamma}}
\newcommand{\Hi}{\ensuremath{\mathcal{H}}}
\newcommand{\Res}[1]{\underset{{#1}}{\mathrm{Res}}}
\newcommand{\ta}[0]{\varphi}
\newcommand{\T}{\mathbb{T}}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\ep}{\epsilon}
\newcommand{\RR}{\mathbb{R}_+\times\mathbb{R}}

\renewcommand{\d}{\mathrm d}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Ai}{Ai} \DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator*{\var}{Var}
\DeclareMathOperator*{\sgn}{sgn}




%%%%%%%%%%%%%%%%%%%%
%Jack's macros
%%%%%%%%%%%%%%%%%%%%

%commands
\newcommand{\prob}{\mathbf{P}}
%\newcommand{\Z}{\mathbb{Z}}
\newcommand{\cE}{\mathcal{E}}
%\newcommand{\cB}{\mathcal{B}}
%\newcommand{\cN}{\mathcal{N}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbR}{\mathbb{R}}


